Increasing Efficiency and Result Reliability of Continuous Benchmarking for FaaS Applications

In a continuous deployment setting, Function-as-a-Service (FaaS) applications frequently receive updated releases, each of which can cause a performance regression. While continuous benchmarking, i.e., comparing benchmark results of the updated and the previous version, can detect such regressions, performance variability of FaaS platforms necessitates thousands of function calls, thus, making continuous benchmarking time-intensive and expensive. In this paper, we propose DuetFaaS, an approach which adapts duet benchmarking to FaaS applications. With DuetFaaS, we deploy two versions of FaaS function in a single cloud function instance and execute them in parallel to reduce the impact of platform variability. We evaluate our approach against state-of-the-art approaches, running on AWS Lambda. Overall, DuetFaaS requires fewer invocations to accurately detect performance regressions than other state-of-the-art approaches. In 98.41% of evaluated cases, our approach provides equal or smaller confidence interval size. DuetFaaS achieves an interval size reduction in 59.06% of all evaluated sample sizes when compared to the competitive approaches.

==> sections/2_background_old.tex <==
\section{Background \& Related Work}
\label{sec:background}

\TP{hier muessen wir noch mal gucken, was wir wirklich brauchen}
\NJ{Formatierung ist derzeit etwas komisch, mit subsubsection und emph teilweise in der gleichen Funktion, aber ab Analysis ist emph der subsubsection untergeordnet.}
\TD{Gefixed, passt es vom Inhalt?}
\TP{unnummerierte sections sind immer noch komisch}
\TP{vom inhalt ist es schon stimmig, muss aber noch etwas glatt gezogen werden damit sich das richtig liest}

\DB{das rumeditieren hier klappt so nicht fuer mich. bitte: neue section in neuer datei erstellen, struktur ueberlegen und dann textfragmente von hier einpflegen und roten faden reparieren. vlt kann tobias da zb dabei helfen. es koennte hier tatsaechlich sinn ergeben, nicht zwischen rel work und background zu differenzieren sondern das als ein gesamtkonzept zu diskutieren, weil die alternativen ja später nicht nur diskutiert sondern umgesetzt und durchgebenchmarkt werden. wer rmit, duet benchmarking etc. sonst noch verwendet hat, koennte dann immer der letzte satz einer subsection sein. also muster: KONZEPT-blablabla-KONZEPT. This has also been used for foo [cite], bar[cite] and foobar[cite]. so wie es jetzt ist, wirkt es etwas durcheinander (und wie tobias weiter unten schreibt, muss man sich nicht zu allen dingen abgrenzen, wenn die nicht konkurrierende ansaetze sind.)}

In this section, we introduce the key concepts required for our approach and briefly highlight important related work.

\subsection{Function-as-a-Service (FaaS)}

FaaS is a popular event-driven model in which developers split their application into functions and host them in a cloud environment~\cite{paper_bermbach2021_cloud_engineering}.
The functions are then able to run based on various triggers, such as events or HTTP calls.
From a developer perspective, FaaS is attractive as it offers a pay-per-use model (rather than the pay-as-provisioned model of traditional cloud infrastructure services) with scale-to-zero and because the entire function lifecycle including failure management and scaling is handled by the platform provider~\cite{bermbach2020using}.




\subsection{Duet Benchmarking}
Duet Benchmarking aims to guarantee resource fairness for both function versions by executing both in parallel.
The artifacts are usually containerized, provided the same amount of resources (CPU, memory, etc.), and then executed in parallel, which also causes occurring uncontrollable factors to influence both versions equally~\cite{bulej2020duet}.
This process enables a fair benchmarking procedure when wanting to efficiently detect performance variation in software application releases.
Duet benchmarking was originally introduced to improve measurement accuracy on cloud instances, but has been extended to other fields~\cite{bulej2020duet}.
More recently it was shown that it is well suited for microbenchmarks, and early findings also showed large improvements with benchmarking suites~\cite{bulej2020duet,bulej2019initial}.
To the best of our knowledge, the duet benchmarking methodology has not been used to evaluate FaaS application releases.
However, published work includes its introduction and evaluation in general cloud benchmarking~\cite{bulej2020duet}, while other papers consider it as a valid remediation step to possibly improve their results~\cite{schirmer2023nightshift}.




\subsubsection*{Analysis}
\TP{die ganze section kann raus, hier reicht ein cite an der ersten stelle wo es benutzt wird}
\TD{David meinte gestern, dass eine Erklärung von Confidence Intervallen und Bootstrapping für die IC2E Audience notwendig wäre}

Performance Change Detection includes the benchmarking and evaluation of application releases to detect significant performance variations. This process is done to ensure that both the user and developer do not experience unexpected side effects.
The user could expect an answer from the application within a certain time period, while the developer has to pay for the additional duration both in local and FaaS environments.

Bootstrapping Percentile Intervals involves the re-sampling of collected values with replacement to calculate confidence intervals for a collection of measurements.
A confidence interval determines the likelihood of a future result from a distribution to be within a bound, the minimum and maximum.
A 99\% confidence interval for example defines a range in which 99\% of future values are likely to be within.
We rely on this methodology in our study as it is commonly used and makes no assumptions about the actual distribution of measurements~\cite{puth2015variety,kalibera2020quantifying}.

\subsection{Related Work}
\TP{ein bisschen tipp zur entscheidung zwischen related work und background: background sind sachen, auf denen deine arbeit aufbaut. related work sind ansaetze, die mit deinem competen (oder bei denen reviewer denken, sie koennten damit competen). du benutzt duet benchmarking und entwickelst es weiter: es ist background. du sagst faasterbench ist unzureichend und schlaegst einen alternativen ansatz vor: es ist related work. jemand macht auch duet benchmarking aber fuer (zb) datenbanken: es ist related work}

Alternative approaches regarding the use of the RMIT benchmarking methodology have been researched, along with the application of duet benchmarking for microbenchmarks.

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{graphs/RMIT.pdf}
    \caption{RMIT Functionality within faasterBench, where a wrapper artifact containing both versions determines a random factor. This random factor decides in which order the functions are run, and the experiment is repeated for several trials.}
    \label{img:rmit}
\end{figure}

In faasterBench, Grambow et al.~implemented the randomized sequential (or RMIT) benchmarking methodology in FaaS. In RMIT, a random factor decides the execution order of the artifacts. The functions are then run in that order, and the order is randomized again. This is repeated for multiple trials, hence the name of randomized multiple interleaved trials~\cite{abedi2017conducting,grambow2023efficiently}.
\cref{img:rmit} highlights how Grambow et al. implemented the RMIT methodology in previous research. Here, they created a wrapper artifact containing both releases, and then called these in an RMIT fashion. The authors showed that RMIT can improve result accuracy and requires fewer results than the traditional approach, where both versions are deployed separately and called independently of one another~\cite{grambow2023efficiently}.

Besides its initial introduction, duet benchmarking has been extended to microbenchmarks by Japke et al.~\cite{japke2023early}. Here, the authors evaluated the use of duet benchmarking based microbenchmarks instead of application benchmarks. Their results showed that these microbenchmarks were able to detect performance issues much earlier than the compared approach, and was also able to detect more fine-grained injected issues.

Our research is not the first to examine performance variation between two or more function updates, with the most recent being one of our previous papers implementing the RMIT methodology to reduce the impact of uncontrollable factors on the result~\cite{grambow2023efficiently}.
Other papers implement an e-divisive algorithm, rely on machine learning, or use microbenchmark suites to detect changes in performance~\cite{daly2020use,grambow2019continuous,toslali2021iter8}.
To the best of our knowledge, we are the first to use duet benchmarking to detect regression in a FaaS environment.



==> sections/3_approach_old.tex <==
\section{Duet Benchmarking FaaS Application Releases}
\label{sec:approach}
\DB{ich bin mir noch nicht ganz im klaren, was das ziel dieser section ist. ich vermute, dass es darum geht, den ansatz vorzustellen, bzw. die anpassungen von duet benchmarking zu beschreiben; das ist aber noch nicht so richtig klar. hier koennte es evtl. sinn ergeben, unterabschnitte fuer issues in vanilla duet benchmarking zu machen und jeweils kurz zu beschreiben, wie die adressiert wurden (vorausgesetzt, dass es mehrere issues gibt). alternativ koennte man mit requirements anfangen und dann beschreiben, wie man die adressiert hat. ein uebersichtsbild ueber das design waere vermutlich auch recht hilfreich -- in dem konkreten fall hier koennte man daher ausnahmsweise auch ueberlegen die impl als eigene subsection ``prototypical implementation'' am ende zu haben. gerade auch weil das tooling mit github actions etc. irgendwie dazugehört und man das super als uebersichtsbild machen kann. das wuerde auch ersparen, dass man bei der eval section als subsections einmal poc und einmal experiments hat und (fast) alles, was bisher subsection ist als subsubsection unter experiments haengen muss.}


\TP{vielleicht bevor wir zu den problemen kommen erst mal zu den ideen die wir haben, warum wir das ueberhaupt machen wollen?}
\TD{Absatz hier drüber eingefügt, um genau das zu besprechen}
Applying duet benchmarking to FaaS artifacts requires several design choices that need to be made before experiments can be run
In this section, we discuss our design that enables duet benchmarking on a public FaaS platform, and what benefits our choices provide.

\subsection{Design Choices}
\DB{nie nur eine subsection haben}
FaaS platforms do not natively support the duet benchmarking methodology, as the degree of control required to run such experiments is higher than what such a service usually provides. 
Function artifacts need to be run on the same instance, share the available memory, but run in parallel on separate cores to correctly implement the procedure.

We decide on running a web server as a FaaS function. 
This allows us to pass configuration options to the server, which ensure both the parallel execution and the distribution of artifacts across separate CPU cores. 
We can use the primary process running on our server to coordinate worker processes, which can then be told to run each artifact in parallel. 
This primary process directly acts as the scheduler, which along with the other configuration options enables duet benchmarking within a FaaS function. 

This FaaS web server is usable within a public cloud environment and can be deployed as a FaaS function there, which brings several benefits along with it. A local deployment would likely not include the uncontrollable factors present in the cloud, and make for highly varying results depending on the execution environment. 
Another option would be to host the function on a cloud instance, but not as a FaaS function. This would be closer to what we are trying to achieve, but performance would likely still differ from what one could expect in an actual FaaS environment. 
Our approach inherently includes the benefit of being usable in a FaaS environment, which also makes our experiment results more comparable with similar approaches. We believe this to the most "FaaS-like" environment possible when wanting to run FaaS duet benchmark experiments. 

As our function is deployable to a public cloud platform, we can also use an action within a deployment pipeline to run fully automated experiments. We can set up the action to monitor the version control system for relevant changes, which then trigger an automatic deployment, benchmark execution, and destruction of duet benchmark experiments. This is also another reason why a local deployment would not suffice, as it would prove difficult to make every possible local environment with compatible with a deployment pipeline. 

Grambow et al. deployed multiple function artifacts in parallel to more quickly complete benchmark experiments, as well as reduce the impact that a 'bad' instance can have on the overall results. As we want experiments to quickly finish, we also make our approach deploy multiple FaaS instances at once, each hosting our duet benchmarking approach. This provides the same benefits as in other research, both reducing the impact of 'bad' instances and reducing the required time for benchmark completion~\cite{grambow2023efficiently}.
\cref{img:systemdesign} shows the simplified design architecture of DuetFaaS (the name of our approach). 
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{graphs/architecture.pdf}
    \caption{Whenever a change in the repository is made, a deployment pipeline uploads the updated and previous version to multiple FaaS instances. Here, both versions are run on separate cores and in parallel to enable duet benchmarking.}
    \label{img:systemdesign}
\end{figure*}
